Verifying the Safety of a Flight-Critical System

This paper describes our work on demonstrating verification technologies on a flight-critical system of realistic functionality, size, and complexity. Our work targeted a commercial aircraft control system named Transport Class Model (TCM), and involved several stages: formalizing and disambiguating requirements in collaboration with do- main experts; processing models for their use by formal verification tools; applying compositional techniques at the architectural and component level to scale verification. Performed in the context of a major NASA milestone, this study of formal verification in practice is one of the most challenging that our group has performed, and it took several person months to complete it. This paper describes the methodology that we followed and the lessons that we learned.

==> safetyCase.tex <==
%!TEX root = main.tex
\section{Safety Case}
\label{sec:safetyCase}

%\subsection{Why semi-formal safety arguments?}

In commercial aviation, the ultimate goal is to certify that a flight-critical system is safe. Software verification is an important part of this process, but is seldom
sufficient when peoples' lives or health are
on the line.  In such cases, a system is often required to be
``certified'', which generally comes down to a government
organization or a company or a person signing off on the system and
saying, in effect, ``We/I certify that this system will not cause
people to be harmed more than once in X hours of operation,'' where X
can be quite large.  (In commercial aviation, this ``X'' may be as
much as a billion -- $10^9$ -- hours of operation.)

Organizations and people, quite naturally, are reluctant to sign off
on such statements unless they are sure the statements are true.
Formal verifications can help alleviate these concerns for parts of a
system, but in the end it is people who must be convinced of the
system's safety.  This is where safety cases may help.


\subsection{Safety Cases -- Background}
\label{subsec:safetycases-background}

%% "A documented body of evidence that provides a convincing and valid
%% argument that a system is adequately safe for a given application
%% in a given environment"


The safety case methodology is a semi-formal way of laying out a
convincing and valid argument, together with the evidence supporting
that argument, that a specific system is sufficiently safe that it can
be used in a given application while operating in a given environment.
All of these caveats are important: the methodology is only
semi-formal, not formal; the arguments only apply to a specific system
(safety arguments are notoriously sensitive to apparently minor
changes in their initial assumptions); even for a fixed system, the
safety properties may change completely in a new environment; a system
is ``sufficiently safe'' only when you know what that term means in
that particular instance; and the safety case must include sufficient
evidence to support the argument.

%% So a safety case can have formal, semi-formal, and heuristic
%% components.  The important thing is that the safety case supports
%% those arguments with convincing (to someone) evidence that clearly
%% demonstrates (to someone) that the desired properties hold.

%% For safety cases, the term ``semi-formal'' implies that the claims,
%% arguments, and evidence for the safety of a system (in a given
%% environment, etc.) are explicitly presented and are convincing to
%% experts in the system's domain.  The arguments are only
%% ``semi-formal'' because, while some parts of the arguments may include
%% rigorous proofs, other parts may be completely heuristic but still be
%% adequately convincing to the experts who must certify the safety of
%% the system(s).  

Several standard ways of presenting these claims, evidence, and
context in a format that enhances the review process and clarifies the
arguments have been developed, including free-form text, ``Claims
Argument Evidence'' (CAE), and ``Goal Structuring Notation'' (GSN).
Similarly, there are many tools to help with building safety cases in
these notations, including ASCE, CertWare, ACCESS, and AdvoCATE.

%% but for this work we have used a standard notation, ``Goal
%% Structuring Notation'' (GSN), and a tool (AdvoCATE) that uses that
%% extension to make the arguments, evidence, and context explicit.

\subsection{Goal Structuring Notation and AdvoCATE}
\label{subsec:gsn-advocate}
In the past, safety case arguments and evidence have been presented
with ad hoc notations, including just plain text (i.e. natural
language) presentations.  But the difficulty has been that the
arguments supporting safety claims were often poorly communicated,
leading to safety claims that were hard to verify.  

For example, \figurename~\ref{fig:text-safety-arg}, taken from
\cite{GSN-Overview}, shows a fragment of a textual safety argument as
used in an actual industrial safety case.  The free-form text in this
example makes it difficult to identify what form of argumentation is
being used or whether the evidence presented is sufficient to
adequately demonstrate that argument.

\begin{figure}[!t]
  \centering
  \begin{small}
  \begin{framed} 
    For hazards associated with warnings, the assumptions of
             [7] Section 3.4 associated with the requirement to
             present a warning when no equipment failure has occurred
             are carried forward. In particular, with respect to
             hazard 17 in section 5.7 [4] that for test operation,
             operating limits will need to be introduced to protect
             against the hazard, whilst further data is gathered to
             determine the extent of the problem.
  \end{framed}
  \end{small}
  \vspace{-0.1in}
  \caption{Textual Safety Argument Fragment}
  \label{fig:text-safety-arg}
\end{figure}

As mentioned above, in response to this lack of clarity a number of
formalisms and tools for using them have been developed, but for this
work we have relied on the Goal Structuring Notation (GSN)
\cite{GSN-Overview} formalism and the AdvoCATE tool \cite{AdvoCATE}.

%gsn-ASafetyArgumenNotation-dsn2004.pdf

\subsubsection{Goal Structuring Notation}
\label{subsubsec:gsn}

A safety case specified with Goal Structuring Notation (GSN)
\cite{GSN-Standard} takes the form of a graph composed of
\emph{elements} (the graph vertices) and \emph{linkages} (the graph
edges) connecting the elements. GSN defines six types of elements and
two types of linkages; for brevity we show only a subset of the GSN
elements in Table~\ref{tab:gsn-sample}.  The full set of element and
linkage types can be found in \cite{GSN-Standard}.

A very small portion of a GSN safety case can be seen in Figure
\ref{fig:gsn-example}.  In this example, the top-level element of the
safety case, G9, is a goal which describes the safety claim being
made, G-120.  The strategy S5 specifies that the goal G9 can be
demonstrated by providing valid safety arguments for each of the
subgoals G12 (that requirement A2 holds) and G14 (that FPA1
holds).  Strategies S7 and S8 say that goals G12 and G14, in turn, can
be demonstrated through formal arguments using the tools described in Section~\ref{sec:verification}.

\begin{table}[ht]
\caption{Sample GSN Element Types}
\centering
\begin{tabular}{ m{0.5in} m{1in} m{1in} }
\hline\\
[-0.1in]
Context&The context in which a Goal is claimed to hold&\includegraphics[width=1in]{figures/Context.eps}\\
\hline\\
[-0.1in]
Goal&A safety claim about the system which must hold&\includegraphics[width=1in]{figures/Goal.eps}\\
\hline\\
[-0.1in]
Strategy&The way a Goal is shown to hold&\includegraphics[width=1in]{figures/Strategy.eps}\\
\hline\\
\end{tabular}
\label{tab:gsn-sample}
\end{table}


%% \subsection{GSN Patterns}

\subsubsection{AdvoCATE}
\label{subsubsec:AdvoCATE}
%% \includegraphics[width=3in]{afcs-p3-rationale-2-simplified.eps}
\begin{figure}[t]
\centering
\includegraphics[height=3.5in]{figures/afcs-p3-rationale-2-simplified-instance-6-3b.eps}
\caption{A Fragment of a GSN Safety Case}
\label{fig:gsn-example}
\end{figure}

Safety cases are typically very large and complex.  In the example we
looked at, a part of the TCM autopilot specified in detail and traced through the GNC system all up all the way through the FARs (see section~\ref{sec:requirements}), the safety case had
several thousand nodes (goals, strategies, etc.).  From this size
alone it can readily be seen that producing detailed and accurate
safety cases by hand is a tedious and error-prone process.

There are a number of tools available for creating safety cases (for
example, \cite{ACCESS,ASCE}), but with most of these tools the process
of creating safety cases is mainly manual: each node must be created
by hand with very limited automation.  On the other hand, the AdvoCATE
\cite{AdvoCATE} tool allows the user to automatically specify common
safety case argument patterns, instantiate those patterns as
(potentially large) pieces of safety cases
(\cite{FormalSafetyCasePatterns}), and then combine those pieces into
a single safety case.


%% \subsection{Results}

%% \subsection{Limitations and Future Work}


\subsection{Safety Case Results and Future Work}
\label{subsec:SCResults}

Although our final safety case contained almost two thousand nodes
derived from close to five hundred requirements, it was produced from
a GSN pattern consisting of fewer than twenty nodes.  This compression
is the result of a limited number of argument types -- the most
important types being argument by direct formal proof (e.g. with PKind
as discussed in Section~\ref{sec:verification}), argument by formal
compositional reasoning over formally proved component goals, and
argument by informal compositional reasoning.  The latter applies to
those cases where at least one of the parent's component goals has not
been formally proven, but can be established to the satisfaction of
the certifying authority by some form of informal reasoning
(e.g. through testing).

Although the safety case for the TCM is quite large, the limited
number of argument types (in GSN terminology, the different
Strategies) and the clearly identified relationships among goals and
subgoals would make it easier for certification authorities to
evaluate evidence, context, and argumentation validity for each of the
goals and to sign off on those goals' satisfaction.

However, our work also points to a limitation of the capabilities of
the version of AdvoCATE used in this case study: its very limited
capability to modularize safety cases.  After all, certifying a
monolithic safety case of several thousand nodes is a daunting
prospect.  Although there are only a limited number of argument types
(Strategies), the sheer number of claims (Goals) can seem
overwhelming.  And our study looked at just a small part of the TCM --
a safety case for the full system would be much larger. It is for
this reason that one of the priorities of the developers of AdvoCATE
is to support modular safety cases as specified in the Goal
Structuring Notation standard~\cite{GSN-Standard} and to investigate
other ways of exploiting and presenting safety case modularity.

AdvoCATE is under constant development and the latest version has many
capabilities beyond those available for the current study.  These
include extensive predefined metadata fields, as well as user-defined
metadata fields.  In the latest version it is possible to annotate
safety case nodes with attributes such as risk (for goal nodes, the
likelihood of not satisfying the goal and severity of the consequences
of non-satisfaction), whether a goal has been formalized or not,
whether a goal is dependent on particular assumptions, and so on.

Based on these fields and other aspects of a safety case, the latest
version of AdvoCATE allows verification tasks (``verify that all leaf
subgoals of a given goal have high-confidence evidence supporting
them''), queries (``find all evidence nodes related to autopilot goal
nodes''), various metrics, sophisticated report generation, and so on.


==> tcm_properties.tex <==
%!TEX root = main.tex
\begin{table*}[!t]
\caption{A summary of verified properties on the TCM.}
\label{tab:tcm_prop}
\centering
\begin{small}
\begin{tabular}{|l|l|l|l|}
\hline
\# & Property &  Assumptions  & Original Requirement\\
\hline
\cellcolor{gray!25}1& \cellcolor{gray!25}G-250 & \cellcolor{gray!25}G-260 & \cellcolor{gray!25}The heading control mode, when selected, sends roll\\
\cellcolor{gray!25}& \cellcolor{gray!25}& \cellcolor{gray!25}
&\cellcolor{gray!25}commands to turn to and maintain the commanded heading. \\
\hline
\cellcolor{gray!25}2&\cellcolor{gray!25}G-110 & \cellcolor{gray!25}G-220,G-260& \cellcolor{gray!25}The guidance system shall be capable of steering to and\\
\cellcolor{gray!25}&\cellcolor{gray!25} &\cellcolor{gray!25}&\cellcolor{gray!25}following a specified heading. \\
\hline
\cellcolor{gray!25}3&\cellcolor{gray!25}G-120 &\cellcolor{gray!25}G-180,A1,A2, & \cellcolor{gray!25}The guidance shall be capable of climbing at a defined rate, to be\\
\cellcolor{gray!25} &\cellcolor{gray!25} &\cellcolor{gray!25} FPA1&\cellcolor{gray!25}limited by minimum and maximum engine performance and airspeeds. \\
\hline
\cellcolor{gray!25}4&\cellcolor{gray!25}G-130& \cellcolor{gray!25}G-180,A1,A2 & \cellcolor{gray!25}The guidance shall be capable of descending at a defined rate, to be\\
\cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25}&\cellcolor{gray!25}limited by minimum and maximum engine performance airspeeds. \\
\hline
\cellcolor{gray!25}5&\cellcolor{gray!25}G-140&\cellcolor{gray!25}G-120,G-200 & \cellcolor{gray!25}The guidance shall be capable of climbing at a specified rate\\
\cellcolor{gray!25} & \cellcolor{gray!25} & \cellcolor{gray!25}
&\cellcolor{gray!25}to a specified altitude, to be limited by maximum engine \\
\cellcolor{gray!25} & \cellcolor{gray!25}&\cellcolor{gray!25} &\cellcolor{gray!25}performance for a set airspeed \\  
\hline
\cellcolor{gray!25}6& \cellcolor{gray!25}G-150& \cellcolor{gray!25}G-180,A1,G-120,&\cellcolor{gray!25}The guidance shall be capable of descending at a specified rate\\
\cellcolor{gray!25} &\cellcolor{gray!25} &\cellcolor{gray!25}A2,G-200 &\cellcolor{gray!25}to a specified altitude, to be limited by maximum engine\\
\cellcolor{gray!25} &\cellcolor{gray!25} &\cellcolor{gray!25} &\cellcolor{gray!25}performance for a set airspeed \\  
\hline
\cellcolor{green!25}7 & \cellcolor{green!25}G-170 (Mode)& \cellcolor{green!25}-- &\cellcolor{green!25}The altitude control shall engage when the altitude control mode \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}is selected and when the FPA control mode is not selected, and when\\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25} &\cellcolor{green!25}there is no manual pitch or manual roll command from the stick.\\
\hline
\cellcolor{green!25}8&\cellcolor{green!25}G-180 (Mode) & \cellcolor{green!25}-- &\cellcolor{green!25}\cellcolor{green!25}The FPA control shall engage when the FPA mode \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}is selected, and when there is no manual pitch or manual roll \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25} &\cellcolor{green!25}command from the stick.\\
\hline
\cellcolor{green!25}9&\cellcolor{green!25}G-100 & \cellcolor{green!25}-- &\cellcolor{green!25}The Guidance system shall be capable of maintaining a steady speed \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}in the normal flight envelope. \\
\hline
\cellcolor{green!25}10&\cellcolor{green!25}G-200 &\cellcolor{green!25}-- &\cellcolor{green!25}If the altitude control is engaged, once the plane is within 250 ft of \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}the commanded altitude, the plane will remain within 250 ft \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}of the commanded altitude. \\
\hline
\cellcolor{green!25}11&\cellcolor{green!25}G-210 (Mode) & \cellcolor{green!25}-- &\cellcolor{green!25}If the FPA control and the altitude control are both selected, the FPA\\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}control will disengage and the altitude control will engage once the\\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25} &\cellcolor{green!25}lane is within 200 ft of the commanded altitude.\\
\hline
\cellcolor{green!25}12&\cellcolor{green!25}G-220 (Mode) & \cellcolor{green!25}-- &\cellcolor{green!25}The heading control shall engage when the heading control mode \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}is selected, and when there is no manual pitch or manual roll \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}command from the stick.\\
\hline
\cellcolor{green!25}13&\cellcolor{green!25}G-230 & \cellcolor{green!25}-- &\cellcolor{green!25}If the altitude control is engaged with no active speed control, \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}the speed control shall engage and the speed command shall synchronize \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25} &\cellcolor{green!25}to the current speed, which shall become the new altitude's target speed.\\
\hline
\cellcolor{green!25}14&\cellcolor{green!25}G-240 &\cellcolor{green!25}--&\cellcolor{green!25}The bank angle limit is established by the Bank Angle Limit Selector.\\
\hline
\cellcolor{green!25}15&\cellcolor{green!25}G-260 (Mode) &\cellcolor{green!25}--&\cellcolor{green!25}When the heading control mode is engaged, roll commands \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}are given to turn in the nearest direction to the selected heading. \\
\hline
\cellcolor{green!25}16&\cellcolor{green!25}G-270 &\cellcolor{green!25}--&\cellcolor{green!25}Manually positioning the thrust levers does not cause \\
\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}&\cellcolor{green!25}autothrottle disengagement. \\
\hline
\cellcolor{green!25}17&\cellcolor{green!25}G-290 &\cellcolor{green!25}--  &\cellcolor{green!25}The autothrottle will be limited by the max and the min throttle.\\
\hline
\cellcolor{red!25}18&\cellcolor{red!25}G-160&\cellcolor{red!25}--  
&\cellcolor{red!25}The guidance function shall be able to automatically deploy spoilers\\
\cellcolor{red!25}&\cellcolor{red!25} &\cellcolor{red!25} &\cellcolor{red!25}to limit speed in a descent, or when a significant reduction in  \\
\cellcolor{red!25} &\cellcolor{red!25} &\cellcolor{red!25} &\cellcolor{red!25}airspeed is requested by the pilot, deactivating at low speed. \\
\hline
\cellcolor{red!25}19&\cellcolor{red!25}G-280 &\cellcolor{red!25}--  
&\cellcolor{red!25}The FCCs shall issue a warning when the commanded altitude\\
\cellcolor{red!25}&\cellcolor{red!25} &\cellcolor{red!25}
&\cellcolor{red!25}disagrees with the stored commanded altitude stored in the FCCs.\\
\hline
\cellcolor{red!25}20&\cellcolor{red!25}G-190 & \cellcolor{red!25}-- &\cellcolor{red!25}If any control surface actuator loses hydraulic pressure, \\
\cellcolor{red!25}&\cellcolor{red!25} &\cellcolor{red!25} &\cellcolor{red!25}the autopilot shall disengage.\\
\hline
\end{tabular}
\end{small}
%\caption{A summary of verified properties on the TCM.}
%\label{fig:tcm_prop}
%\end{figure*}
\end{table*}
